Model-based Adversarial Meta-Reinforcement Learning

Meta-reinforcement learning (meta-RL) aims to learn from multiple training tasks the ability to adapt efficiently to unseen test tasks. Despite the success, existing meta-RL algorithms are known to be sensitive to the task distribution shift. When the test task distribution is different from the training task distribution, the performance may degrade significantly. To address this issue, this paper proposes Model-based Adversarial Meta-Reinforcement Learning (AdMRL), where we aim to minimize the worst-case sub-optimality gap -- the difference between the optimal return and the return that the algorithm achieves after adaptation -- across all tasks in a family of tasks, with a model-based approach. We propose a minimax objective and optimize it by alternating between learning the dynamics model on a fixed task and finding the adversarial task for the current model -- the task for which the policy induced by the model is maximally suboptimal. Assuming the family of tasks is parameterized, we derive a formula for the gradient of the suboptimality with respect to the task parameters via the implicit function theorem, and show how the gradient estimator can be efficiently implemented by the conjugate gradient method and a novel use of the REINFORCE estimator. We evaluate our approach on several continuous control benchmarks and demonstrate its efficacy in the worst-case performance over all tasks, the generalization power to out-of-distribution tasks, and in training and test time sample efficiency, over existing state-of-the-art meta-RL algorithms.

==> impact.tex <==
\section*{Broader Impact}

Meta-reinforcement learning has potential positive impact in real-life applications such as robotics. For example, in robotic assembly tasks, it is expensive and time-consuming to have engineers hand-produce controllers for each new configuration of parts; meta-RL allows for rapid development of controllers for new tasks, efficiently enabling greater variation and customizability in the manufacturing process.

Our method makes meta-RL more practical in several ways:
\begin{enumerate}
    \item By vastly improving the sample efficiency of meta-training compared to previous approaches, we lower the barrier to entry.
    \item Directly optimizing worst-case performance reduces the chance of a catastrophic failure.
    \item Zero-shot adaptation already produces a fairly strong policy, thereby improving safety in settings where an untrained policy is prone to cause damage.
\end{enumerate}

On the other hand, there are potential risks as well. Increased automation can reduce the demand for labor in certain industries, thereby impacting job availability.
